Reducing Human-Robot Goal State Divergence with Environment Design

One of the most difficult challenges in creating successful human-AI collaborations is aligning a robot's behavior with a human user's expectations. When this fails to occur, a robot may misinterpret their specified goals, prompting it to perform actions with unanticipated, potentially dangerous side effects. To avoid this, we propose a new metric we call Goal State Divergence $\mathcal{(GSD)}$, which represents the difference between a robot's final goal state and the one a human user expected. In cases where $\mathcal{GSD}$ cannot be directly calculated, we show how it can be approximated using maximal and minimal bounds. We then input the $\mathcal{GSD}$ value into our novel human-robot goal alignment (HRGA) design problem, which identifies a minimal set of environment modifications that can prevent mismatches like this. To show the effectiveness of $\mathcal{GSD}$ for reducing differences between human-robot goal states, we empirically evaluate our approach on several standard benchmarks.

==> 5-0-method-main.tex <==

\section{Design to Reduce Goal State Divergence}
As discussed, the mismatch between the human's perception of the robot's capabilities/state and the reality could lead to users misspecifying their objective, potentially resulting in unanticipated outcomes. Earlier, we saw this happen when a human instructed a robot to water plants in a greenhouse, and rather than doing what they expected -- using a water pail to care for them -- the robot instead used a hose. This misspecification led to the robot unintentionally spraying heat lamps with water, triggering a fire in the process. To develop methods that can account for and avoid such unintended outcomes, we first need to develop metrics to quantify the degree mismatch. Specifically, we will start by looking at pairs of states.
\begin{defn}
\textit{Given any two states, $s^1, {s}^2$, state divergence (SD) is defined as the symmetric difference between their respective fluents, i.e.:}
\begin{align*} 
\mathcal{SD}(s^1, s^2) = s^1 \Delta \  s^2 
\end{align*}
\end{defn}

However, in this paper, we are not interested in just measuring the difference between two arbitrary states, but the goal state expected by the user and the goal state that the robot can achieve. This requires us to measure the difference in states achievable across models:
\begin{defn}
\textit{For a pair of models that are not necessarily distinct, $\mathcal{M}^1$ and $\mathcal{M}^2$, let $\pi_1$ be a valid plan in $\mathcal{M}^1$, and $\pi_2$ be a valid plan in $\mathcal{M}^2$. Given this, goal state divergence ($\GSD$) of the plans is defined as the state divergence between the final goal state of these two plans, i.e:}
\begin{align*} 
\GSD(\pi_1, \mathcal{M}^1, \pi_2, \mathcal{M}^2) = \mathcal{SD} ( \mathcal{T}_{\mathcal{M}^1}(I^1, \pi_1) \ , \ \mathcal{T}_{\mathcal{M}^2}(I^2, \pi_2) ) 
\end{align*} 
\end{defn}


In our setting, these two models correspond to the robot model $\mathcal{M^R} = \langle \mathcal{D^R}, \mathcal{P^R}\rangle$, and the human's model of the robot and the task $\mathcal{M^H}= \langle \mathcal{D^H}, \mathcal{P^H}\rangle$. 
We are specifically, looking at cases where the robot is trying to exactly follow the instructions specified by the user and thus we have  $\mathcal{G}^H = \mathcal{G}^R$.
For simplifying the notations, we will additionally assume that the initial state estimates are the same \footnote{It is worth noting that we can easily extend our work to support differences in initial states.}.
As such, the difference between the human expectation and the robot's final goal state arises because of differences between  $\mathcal{D^H}$ and $\mathcal{D^R}$.
In this paper, we will focus our attention on cases where the robot is capable of computing the optimal plan and thus chooses a plan $\pi^R \in \Pi^*_R$. Now as for the human plan, let $\pi^H$ be the plan selected by the human. Now there are two main challenges to calculating $\GSD$ for this setting, namely the knowledge of the human model and the plan $\pi^H$. Thankfully, there are a number of works that have looked at the former problem (cf. \cite{}), in addition to all the works in learning planning models in general. Also, under many structured settings the human model may be known beforehand. For example, in the greenhouse case, if the user has been working with a previous model of the robot, their beliefs about the robot would be heavily influenced by the capabilities of the previous model. So through this paper, we will make the assumption that the model is given to us. However, even with the model known, the exact plan the human chooses may not be known beforehand. This means that rather than trying to exactly estimate $\GSD$, we will consider approximations. The first approximation we will consider is the worst-case approximation, where we will look at the maximum divergence possible between an expected human goal state and what the robot can achieve, more formally,
\begin{defn}
\textit{For two given models, $\mathcal{M}^1$, $\mathcal{M}^2$, the worst-case or maximal goal state divergence ($\MxGD$) is given by the cardinality of the maximum goal state divergence possible between all executable plans in $\mathcal{M}^1$, $\Pi_{{\mathcal{M}^1}}$, and $\mathcal{M}^2$, i.e,:}
\begin{align*}
\MxGD(\mathcal{M}^1, \mathcal{M}^2) = \max_{ \pi \in \Pi_{{\mathcal{M}^1}}, \pi' \in \Pi_{{\mathcal{M}^2}} }(|\GSD(\pi_1, \mathcal{M}^1, \pi_2, \mathcal{M}^2)|) 
\end{align*}
\end{defn}

This brings us to our first proposition which states that $\MxGD$ is guaranteed to be an upper bound of the true goal state divergence.
\begin{prop}
\label{prop:upper}
    For the robot and human model pair $\mathcal{M}^R$ and $\mathcal{M}^H$, the maximal goal state divergence is guaranteed to be greater than the goal state divergence for the human plan $\pi^H$ and the robot plan $\pi^R$, i.e.,  $\MxGD(\mathcal{M}^H, \mathcal{M}^R) \geq |\GSD(\mathcal{M}^H, \pi^H, \mathcal{M}^R, \pi^R)|$.
\end{prop}
The validity of the above proposition can be trivially proven from the definition of $\MxGD$. From the proposition, we can assert that one way to reduce goal-state divergence is to reduce $\MxGD$. Especially, if we can reduce $\MxGD$ to zero, we are guaranteed that $\GSD$, will be an empty set. 

However, $\MxGD$ could be a loose upper bound, and reducing $\MxGD$ will not necessarily always reduce $\GSD$. Another approximation, we could use is the lower bound on $\GSD$. Now we define this measure similar to $\MxGD$, but now focusing on minimizing the divergence.

\begin{defn}
\textit{For two given models, $\mathcal{M}^1$, $\mathcal{M}^2$, the best-case or minimal goal state divergence ($\MnGD$) is given by the cardinality of the minimum goal state divergence possible between all executable plans in $\mathcal{M}^1$, $\Pi_{{\mathcal{M}^1}}$, and $\mathcal{M}^2$, i.e,:}
\begin{align*}
\MnGD(\mathcal{M}^1, \mathcal{M}^2) = \min_{ \pi \in \Pi_{{\mathcal{M}^1}}, \pi' \in \Pi_{{\mathcal{M}^2}} }(|\GSD(\pi_1, \mathcal{M}^1, \pi_2, \mathcal{M}^2)|) 
\end{align*}
\end{defn}

Similar to Proposition \ref{prop:upper}, we can assert that $\MnGD$ provides us a lower bound.
\begin{prop}
\label{prop:upper}
    For the robot and human model pair $\mathcal{M}^R$ and $\mathcal{M}^H$, the minimal goal state divergence is guaranteed to be less than or equal to the goal state divergence for the human plan $\pi^H$ and the robot plan $\pi^R$, i.e.,  $\MnGD(\mathcal{M}^H, \mathcal{M}^R) \leq |\GSD(\mathcal{M}^H, \pi^H, \mathcal{M}^R, \pi^R)|$.
\end{prop}

Now we can try to characterize our unknown $\GSD$, using this upper bound, lower bound, and the gap between the two (i.e., $\MxGD(\mathcal{M}^H, \mathcal{M}^R) - \MnGD(\mathcal{M}^H, \mathcal{M}^R)$). 

However, note that the definitions provided above are still quite relaxed in the plans being considered.
By considering the space of all plans we are effectively considering a much larger space of models than one that would ever be expected by a human or executed by the robot.
This will result in weaker bounds than what might be effective. For example, in the running example discussed above, regardless of where you place the hose there will always be a plan where the robot could go fetch the hose and spray the plants. Thus if one were to make changes to the model based purely on these metrics, only removing the hose from the setting completely could result in a setting where the use of the hose is not considered as part of one of the possible outcomes.


As discussed, for the robot plan, we can effectively restrict the space of plans to just the optimal plans. However, to make assertions about the possible human plans, we will need to associate a decision-making model with the human. A popular option that is widely used in human-AI interaction literature is the noisy-rational model, where the likelihood of the human choosing a plan is given as
\[P(\pi) \propto e^{-\beta \times c(\pi)}\]
Where $\beta$ is a parameter called the rationality parameter. Now we can only consider plans that are above some probability threshold $\epsilon$. For any such probability threshold, there will be a corresponding cost value $C_{\epsilon}$, such that for any plan $\pi$, where $c(\pi) > C_{\epsilon}$, you will have $P(\pi) < \epsilon$. We will denote the corresponding upper and lower bounds of $\GSD$, where the plan spaces are bounded as described above as $\MxGDstr$ and $\MnGDstr$. Note that limiting the robot's plans to optimal plans already ensures that the design illustrated in Figure \ref{fig:fib} (C/D) will result in the expected outcome.

Now with the basic setting and metrics in place, we are ready to finally define the design problem.

\begin{defn}
\textit{A \textbf{human-robot goal alignment (HRGA)} design problem is characterized by the tuple, $\mathcal{DP} = \langle \mathcal{M^R}, \mathcal{M^H}, \mathbb{U}, \Lambda, \mathcal{C} \rangle$, where:}

\begin{itemize}
\item $\mathcal{D^R}$, $\mathcal{D^H}$, are initial robot and human models.
\item $\mathbb{U}$ is the set of available design modifications or model updates, which may be made to our system inputs i.e. the state space, action preconditions, action effects, action costs, initial state, and goal.
\item $\Lambda : \mathbb{M} \times \mathbb{U} \rightarrow \mathbb{M}$ is the transition function over a space of possible models in an optimal plan alignment problem, which produces an updated problem once modifications have been applied.
\item $\mathcal{C}$ is an additive cost function that maps each design modification in $\mathbb{U}$ to a cost. 

\end{itemize}
\end{defn}

Now one could define various classes of solutions based on the metrics we have described above. The most basic one we can describe is one where we will try to minimize the upper bound while requiring the lower bound to be set to zero and we place a budget on the number of design modifications that can be performed.
\begin{defn}
\textit{A  $k$-bounded minimal solution to $\mathcal{DP}$ is a subset of modifications $\xi$ which minimize the average $\MxGD$ measure for the instance $\mathcal{P}$ as follows:}
\begin{align*} 
\xi^* = \operatorname*{argmin}_{ \xi \in 2^\mathbb{U}} \sum_{\mathcal{P} \in \mathbb{P}}\MxGD(\mathcal{M_{\xi}^{R}}, \mathcal{M_\xi^{H}}) \\
\textrm{Such that }\MnGD=0 \textrm{ and } C(\xi^*) \leq k.
\end{align*}
Where $\mathcal{M_{\xi}^{R}} = \Lambda(\mathcal{M^R} \xi)$ and $\mathcal{M_{\xi}^{H}} = \Lambda(\mathcal{M^H}, \xi)$
\end{defn}

We can quickly form variations of the design objectives by replacing $\MxGD$ and $\MnGD$, with $\MxGDstr$ and $\MnGDstr$. Additionally, in many cases, the design might need to consider a set of possible problem instances. In such cases, the above definition could be replaced with the max, min, or average of the value across the instances.



==> 5-1-algo-old.tex <==
\begin{algorithm}[tbp!]
\caption{An algorithm for a HRGA design problem}
\label{algo1}
\vspace{2pt} 
\begin{algorithmic}[1]

%\textbf{Input}: $\mathcal{DP} = \langle \mathcal{M^R}, \mathcal{M^H}, \mathbb{U}, \Lambda, \mathcal{C} \rangle$\newline

%\textbf{Output}: $\mathcal{M^\lambda}=\langle \mathcal{D^\lambda}, \mathcal{I^\lambda}, \mathcal{T^\lambda}, \mathcal{G^\lambda}, c^\lambda\rangle$\newline

\FOR{budget $\tau$}\\

\State $design\_completed \gets False$\newline
\State $found\_designs \gets \{\}$\newline
\State $best\_designs \gets None$\newline
\State $best\_divergence \gets 10000000$\newline

\WHILE{$design\_completed$ is $false$}\newline
    
    \State{$D^\lambda, P^\lambda\gets MinGSD(\mathcal{M^R}, \mathcal{M^H}, design\_count, found\_designs)$} %causing problems
    
    \State{$ \pi^\lambda, C\gets GetPlan(D^\lambda, P^\lambda)$}%causing problems
    
    \IF{$\pi^\lambda$ length is $0$}\newline
        \State $ design\_completed\gets True $
    \ELSE
        \State $\mathbb{U} = \{\}$\newline %design_set assigned empty set
        \FOR{$a_i^\lambda$ in $\pi^\lambda$}
            %\IF{$"design\_act\_"$ in $a_i^\lambda$}
            \IF{$a_i^\lambda$ is a design action}
                %\STATE{$design\_set.add(action.split("\_act\_")[1])$}
                \STATE{Add $a_i^\lambda$ to $\mathbb{U}$}
            \ENDIF
        \ENDFOR
    
        \State{$ A^{\kappa-} \gets []$}
        %\FOR{$A^\lambda$ in $\pi^\lambda$}
        \FOR{$a_i^\lambda$ in $\pi^\lambda$}
            %\IF{$"check\_disagree\_act\_"$ in $a_i^\lambda$}
            \IF{$a_i^\lambda$ is a check disagreement action}
                \STATE Append $a_i^\lambda$ to $A^{\kappa-}$
            \ENDIF
        \ENDFOR \newline
        \State Append $\mathbb{U}$ to $found\_designs$

        \State{$D^\lambda, P^\lambda\gets MaxGSD(\mathcal{M^R}, \mathcal{M^H}, \mathbb{U}, \tau)$} %causing problems
        \State{$ \pi^\lambda, C\gets GetPlan(D^\lambda, P^\lambda)$} %causing problems

        %\IF{$len(\pi^\lambda) == 0$}\newline
        \IF{$\pi^\lambda$ length is $0$}\newline
            \State $exit(0)$ 
        \ENDIF

        \State{$ A^{\kappa-} \gets []$}
        \FOR{$a_i^\lambda$ in $\pi^\lambda$}
            %\IF{$"check\_disagree\_act\_"$ in $a_i^\lambda$}
            %\IF{$a_i^\lambda$ in $A^\kappa_{f_i}$}
             \IF{$a_i^\lambda$ is a check disagreement action}
                \State Append $a_i^\lambda$ to $A^{\kappa-}$
            \ENDIF
        \ENDFOR

        \IF{$best\_divergence > len(A^{\kappa-})$}
            \State $best\_divergence \gets len(A^{\kappa-})$\newline
            \State $best\_designs \gets \mathbb{U}$
        \ENDIF
    \ENDIF
\ENDWHILE
\ENDFOR
\end{algorithmic}
\end{algorithm}

==> 6-1_table_backup.tex <==
\begin{table*}[h]
\small
\centering
\setlength\tabcolsep{3pt}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Domain &
  \texttt{Main} &
 \texttt{Main-fl} &
\texttt{Naive} &
\texttt{$\MnGD$} & 
\texttt{$\MnGD$ with Design} &
\texttt{$\MxGD$}\\ \hline
\multirow{5}{*}{Blocksworld}&77.9057	$\pm$	2.5187	&	79.4784	$\pm$	3.6204	&	395.1341	$\pm$	1.7968 & 12.2577 $\pm$	12.2577 & 12.0809	$\pm$	0.0779 & 11.2091 $\pm$	1.1940\\
&77.0713	$\pm$	1.0263	&	77.2801	$\pm$	2.3206	&	389.6741	$\pm$	7.3767 & 12.2794 $\pm$	12.2794 & 11.5832	$\pm$	0.9132 & 13.9546 $\pm$	1.1583\\
&124.2159	$\pm$	36.1064	&	129.9057	$\pm$	33.6354	&	478.7145	$\pm$	38.2897 & 11.9615 $\pm$	11.9615 & 12.9646 $\pm$	1.3855 & 36.6411 $\pm$	4.1236\\
&98.1436	$\pm$	3.8912	&	103.6868	$\pm$	1.9262	&	425.1810	$\pm$	4.4099 & 12.2794 $\pm$	12.2794 & 12.8272	$\pm$	0.1673 & 35.3121 $\pm$	0.6635\\
&136.0833	$\pm$	18.3803	&	144.8098	$\pm$	19.3280	&	479.9484	$\pm$	5.8157 & 12.4268 $\pm$	12.4268 & 12.5032	$\pm$	0.0115 & 23.3231 $\pm$	16.3454\\ \hline
\multirow{5}{*}{Logistics}&34.6680	$\pm$	0.5156	&	\textcolor{red}{35.24$\pm$0.94} 	& \textcolor{red}{54.39 $\pm$ 0.87} & 0.8525	$\pm$	0.8525 & 0.9176 $\pm$	0.0136 & 30.2777 $\pm$	1.0289\\
&33.7620	$\pm$	0.4367	&	35.7405	$\pm$	0.4808	&	58.2292	$\pm$	0.0179 & 0.8958 $\pm$	0.8958 & 0.9108 $\pm$	0.0217 & 27.1010 $\pm$	0.0283\\
&33.1861	$\pm$	0.4121	&	34.5544	$\pm$	0.2724	&	57.5689	$\pm$	0.0535 & 0.8992 $\pm$ 0.8992 & 0.9136 $\pm$	0.0018 & 27.8368	$\pm$	0.1676\\
&35.7079	$\pm$	0.5031	&	36.8395	$\pm$	0.7901	&	60.1560	$\pm$	0.8580 & 0.9255 $\pm$	0.9255 & 0.9127 $\pm$	0.0066 & 29.6226 $\pm$	0.0401\\
&34.2042	$\pm$	0.8265	&	35.6552	$\pm$	0.1847	&	57.7684	$\pm$	0.2866 & 0.8922 $\pm$	0.8922 & 0.9043 $\pm$	0.0152 & 27.1590 $\pm$	0.0986\\  \hline
\multirow{5}{*}{Zenotravel}&5.7560	$\pm$	0.0559	&	6.1046	$\pm$	0.0374 	&	28.1113	$\pm$	0.0958 & 0.8737 $\pm$	0.8737 & 0.8921	$\pm$	0.0016 & 0.8458 $\pm$	0.0001\\
&5.8318	$\pm$	0.0279	&	6.2106	$\pm$	0.0133	&	28.2848	$\pm$	0.0090 & 0.8758 $\pm$	0.8758 & 0.9027 $\pm$	0.0064 & 0.8538 $\pm$	0.0026\\
&7.7368	$\pm$	0.0564	&	8.2782	$\pm$	0.0239	&	35.8196	$\pm$	0.0376 & 1.1092 $\pm$	1.1092 & 1.1462 $\pm$	0.0158 & 1.1923 $\pm$	0.0001\\
&7.9403	$\pm$	0.0612	&	8.0233	$\pm$	0.2641	&	36.4870	$\pm$	0.0532 & 1.1389 $\pm$	1.1389 & 1.1742 $\pm$	0.0094 & 1.2598	$\pm$	0.0048\\
&10.1786	$\pm$	1.1797	&	11.3186	$\pm$	0.1412	&	51.0039	$\pm$	0.3473 & 1.0913 $\pm$	1.0913 & 1.6093 $\pm$	0.0267 & 1.6258 $\pm$	0.0062\\  \hline
\multirow{5}{*}{Elevator}& 4.3291	$\pm$	0.0156	&	4.6213	$\pm$	0.0077	&	21.9475	$\pm$	0.0932 & 0.6773 $\pm$	0.6773  & 0.7024	$\pm$	0.0006 & 0.6607 $\pm$	0.0039\\
&4.7732	$\pm$	0.0047	&	5.0510	$\pm$	0.0127	&	23.5855	$\pm$	0.0707 & 0.7370 $\pm$	0.7370 & 0.7779 $\pm$	0.0047 & 0.7122 $\pm$	0.0013\\
&4.7612	$\pm$	0.0015	&	5.0957	$\pm$	0.0139	&	23.7161	$\pm$	0.0054 & 0.7420 $\pm$	0.7420 & 0.7740 $\pm$	0.0028 & 0.7125 $\pm$	0.0027\\
&4.7666	$\pm$	0.0038	&	5.0506	$\pm$	0.0369	&	23.5519	$\pm$	0.0685 & 0.7371 $\pm$	0.7371 & 0.7751 $\pm$	0.0006 & 0.7147 $\pm$	0.0034\\
&4.7668	$\pm$	0.0062	&	5.0245	$\pm$	0.0076	&	23.6539	$\pm$	0.0429 & 0.7125 $\pm$	0.7125 & 0.7758 $\pm$	0.0008 & 0.7137 $\pm$	0.0019\\  \hline
\multirow{5}{*}{Depot}&37.8871	$\pm$	0.1226	&	40.8593	$\pm$	1.9585	&	189.1806	$\pm$	11.4726 & 5.8486 $\pm$	5.8486 & 5.4597 $\pm$ 0.7661 & 5.2322 $\pm$	0.2345\\
&88.1976	$\pm$	2.5745	&	88.8184	$\pm$	3.8472	&	457.3999	$\pm$	6.1602 & 13.3659 $\pm$	13.3659 & 14.5224 $\pm$	0.6518 & 15.7344 $\pm$	0.3281\\
&85.5790	$\pm$	2.5697	&	90.1610	$\pm$	2.9081	&	450.7367	$\pm$	2.0915 & 13.2757 $\pm$	13.2757 & 13.9644 $\pm$	0.1242 & 16.8631 $\pm$	0.9195\\
&86.5167	$\pm$	0.4087	&	91.4319	$\pm$	1.3791	&	457.7135	$\pm$	5.9022 & 13.4442 $\pm$	13.4442 & 15.1228 $\pm$	0.2203 & 15.4043 $\pm$	0.1471\\
&87.4827	$\pm$	0.1825	&	92.0831	$\pm$	3.0986	&	452.2125	$\pm$	1.7390 & 14.5647 $\pm$	14.5647 & 14.7178 $\pm$	0.0339 & 15.4332 $\pm$	0.1933\\
  \hline
  \end{tabular}
  \caption{The average and standard deviation time taken by each method compared to each baseline in seconds per instance. The first three columns respectively present the time taken by our method, a variation of our method that doesn't enforce ordering, and a baseline that iterates over possible designs. The final three columns report the average time taken to compute the lower bound of \GSD, lower bound with design, and upper bound.}
  %\caption{The overall time taken by our method compared to each of the baselines. }
  \label{tab1}
  \end{table*}

%Our primary metric is the time taken by each approach. Accordingly, Table 1 presents the average and standard deviation time in seconds taken per each instance reported.


==> AAAI-HEADER.tex <==

\usepackage[submission]{aaai23}  % DO NOT CHANGE THIS
\usepackage{times}  % DO NOT CHANGE THIS
\usepackage{helvet}  % DO NOT CHANGE THIS
\usepackage{courier}  % DO NOT CHANGE THIS
\usepackage[hyphens]{url}  % DO NOT CHANGE THIS
\usepackage{graphicx} % DO NOT CHANGE THIS
\urlstyle{rm} % DO NOT CHANGE THIS
\def\UrlFont{\rm}  % DO NOT CHANGE THIS
\usepackage{natbib}  % DO NOT CHANGE THIS AND DO NOT ADD ANY OPTIONS TO IT
\usepackage{caption} % DO NOT CHANGE THIS AND DO NOT ADD ANY OPTIONS TO IT
\frenchspacing  % DO NOT CHANGE THIS
\setlength{\pdfpagewidth}{8.5in} % DO NOT CHANGE THIS
\setlength{\pdfpageheight}{11in} % DO NOT CHANGE THIS
%
% These are recommended to typeset algorithms but not required. See the subsubsection on algorithms. Remove them if you don't have algorithms in your paper.
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{multirow}
\usepackage{amsfonts} 

%
% These are are recommended to typeset listings but not required. See the subsubsection on listing. Remove this block if you don't have listings in your paper.
\usepackage{newfloat}
\usepackage{listings}
\DeclareCaptionStyle{ruled}{labelfont=normalfont,labelsep=colon,strut=off} % DO NOT CHANGE THIS
\lstset{%
	basicstyle={\footnotesize\ttfamily},% footnotesize acceptable for monospace
	numbers=left,numberstyle=\footnotesize,xleftmargin=2em,% show line numbers, remove this entire line if you don't want the numbers.
	aboveskip=0pt,belowskip=0pt,%
	showstringspaces=false,tabsize=2,breaklines=true}
\floatstyle{ruled}
\newfloat{listing}{tb}{lst}{}
\floatname{listing}{Listing}
%
% Keep the \pdfinfo as shown here. There's no need
% for you to add the /Title and /Author tags.
\pdfinfo{
/TemplateVersion (2023.1)
}

% DISALLOWED PACKAGES
% \usepackage{authblk} -- This package is specifically forbidden
% \usepackage{balance} -- This package is specifically forbidden
% \usepackage{color (if used in text)
% \usepackage{CJK} -- This package is specifically forbidden
% \usepackage{float} -- This package is specifically forbidden
% \usepackage{flushend} -- This package is specifically forbidden
% \usepackage{fontenc} -- This package is specifically forbidden
% \usepackage{fullpage} -- This package is specifically forbidden
% \usepackage{geometry} -- This package is specifically forbidden
% \usepackage{grffile} -- This package is specifically forbidden
% \usepackage{hyperref} -- This package is specifically forbidden
% \usepackage{navigator} -- This package is specifically forbidden
% (or any other package that embeds links such as navigator or hyperref)
% \indentfirst} -- This package is specifically forbidden
% \layout} -- This package is specifically forbidden
% \multicol} -- This package is specifically forbidden
% \nameref} -- This package is specifically forbidden
% \usepackage{savetrees} -- This package is specifically forbidden
% \usepackage{setspace} -- This package is specifically forbidden
% \usepackage{stfloats} -- This package is specifically forbidden
% \usepackage{tabu} -- This package is specifically forbidden
% \usepackage{titlesec} -- This package is specifically forbidden
% \usepackage{tocbibind} -- This package is specifically forbidden
% \usepackage{ulem} -- This package is specifically forbidden
% \usepackage{wrapfig} -- This package is specifically forbidden
% DISALLOWED COMMANDS
% \nocopyright -- Your paper will not be published if you use this command
% \addtolength -- This command may not be used
% \balance -- This command may not be used
% \baselinestretch -- Your paper will not be published if you use this command
% \clearpage -- No page breaks of any kind may be used for the final version of your paper
% \columnsep -- This command may not be used
% \newpage -- No page breaks of any kind may be used for the final version of your paper
% \pagebreak -- No page breaks of any kind may be used for the final version of your paperr
% \pagestyle -- This command may not be used
% \tiny -- This is not an acceptable font size.
% \vspace{- -- No negative value may be used in proximity of a caption, figure, table, section, subsection, subsubsection, or reference
% \vskip{- -- No negative value may be used to alter spacing above or below a caption, figure, table, section, subsection, subsubsection, or reference

\setcounter{secnumdepth}{0} %May be changed to 1 or 2 if section numbers are desired.

% The file aaai23.sty is the style file for AAAI Press
% proceedings, working notes, and technical reports.
%

% Title

% Your title must be in mixed case, not sentence case.
% That means all verbs (including short verbs like be, is, using,and go),
% nouns, adverbs, adjectives should be capitalized, including both words in hyphenated terms, while
% articles, conjunctions, and prepositions are lower case unless they
% directly follow a colon or long dash



\author{
    %%Authors
    %% All authors must be in the same font size and format.
    %Written by AAAI Press Staff\textsuperscript{\rm %1}\thanks{With help from the AAAI Publications %Committee.}\\
    % AAAI Style Contributions by Pater Patel Schneider,
    % Sunil Issar,\\
    % J. Scott Penberthy,
    % George Ferguson,
    % Hans Guesgen,
    % Francisco Cruz\equalcontrib,
    % Marc Pujol-Gonzalez\equalcontrib
}
\affiliations{
    %%Afiliations
    %\textsuperscript{\rm 1}Association for the Advancement of %Artificial Intelligence\\
    %% If you have multiple authors and multiple affiliations
    %% use superscripts in text and roman font to identify %them.
    %% For example,

    %% Sunil Issar, \textsuperscript{\rm 2}
    %% J. Scott Penberthy, \textsuperscript{\rm 3}
    %% George Ferguson,\textsuperscript{\rm 4}
    %% Hans Guesgen, \textsuperscript{\rm 5}.
    %% Note that the comma should be placed BEFORE the %superscript for optimum readability

    %1900 Embarcadero Road, Suite 101\\
    %Palo Alto, California 94303-3310 USA\\
    %% email address must be in roman text type, not monospace %or sans serif
    %publications23@aaai.org
%
% See more examples next
}

%Example, Single Author, ->> remove \iffalse,\fi and place them surrounding AAAI title to use it
\iffalse
\title{My Publication Title --- Single Author}
\author {
    Author Name
}
\affiliations{
    Affiliation\\
    Affiliation Line 2\\
    name@example.com
}
\fi

\iffalse
%Example, Multiple Authors, ->> remove \iffalse,\fi and place them surrounding AAAI title to use it
\title{My Publication Title --- Multiple Authors}
\author {
    % Authors
    First Author Name,\textsuperscript{\rm 1}
    Second Author Name, \textsuperscript{\rm 2}
    Third Author Name \textsuperscript{\rm 1}
}
\affiliations {
    % Affiliations
    \textsuperscript{\rm 1} Affiliation 1\\
    \textsuperscript{\rm 2} Affiliation 2\\
    firstAuthor@affiliation1.com, secondAuthor@affilation2.com, thirdAuthor@affiliation1.com
}
\fi


% REMOVE THIS: bibentry
% This is only needed to show inline citations in the guidelines document. You should not need it and can safely delete it.
\usepackage{bibentry}
% END REMOVE bibentry




%\newtheorem{example}{Example}
\newtheorem{theorem}{Theorem}
\usepackage{subcaption}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{mathtools}

==> comments.tex <==
\newcount\Comments
\Comments=1
\usepackage{xcolor}
\definecolor{darkgreen}{rgb}{0,0.7,0}

\newcommand{\kibitz}[2]{\ifnum\Comments=1{\color{#1}{#2}}\fi}

\newcommand{\todo}[1]{\kibitz{red}{[todo: #1]}}
\newcommand{\sk}[1]{\kibitz{blue}{[sk: #1]}}
\newcommand{\ga}[1]{\kibitz{green}{[ga: #1]}}

